Work Agents: Systems, Capabilities, and Optimization

As foundation models evolve from information generation to digital work execution, agents are increasingly capable of completing complex tasks across tools, applications, and workflows. However, existing research lacks a unified perspective on how agents reliably accomplish delegated work. To address this gap, we present a work-centric, system-level perspective that views work agents as systems combining foundation models and runtime harnesses to execute tasks in stateful workspaces and deliver verifiable outcomes. We introduce two complementary dimensions, work persistence and work openness, to characterize working conditions, and classify digital work into five forms according to task scope and organization. Building on this framework, we identify five core capability families required for reliable work execution and examine approaches to model optimization, harness optimization, and their joint optimization. We further analyze existing evaluation methods and metrics from the perspective of work outcomes. Finally, we discuss future research directions, including sustained work delegation, adaptation to open environments, and the interaction between work execution and capability improvement. This paper provides a unified framework for understanding, optimizing, and evaluating work agents, supporting the development of systems capable of delivering reliable, verifiable, and practically valuable work outcomes.

==> figures/cover-variants/cover-reference-pins.tex <==
% Quiet upper page, retained footer ribbons, and explicit work-scope semantics.
\input{figures/cover-variants/cover-workscope-symbols.tex}
\input{figures/cover-variants/cover-scope-gradient.tex}
\usetikzlibrary{fadings,decorations.text}
\RequirePackage[outline]{contour}
% PGF inserts \relax between its text-format prefix and each character.
% Outline each glyph, rather than covering the paper ribbons with a label box.
\def\CoverScopeLetterHalo\relax#1{%
  \contourlength{0.45pt}\contour{white}{#1}%
}
\tikzfading[name=coverScopeFooterFade,
  top color=transparent!0,bottom color=transparent!100]
\definecolor{coverPinBlue}{HTML}{098BD0}
\definecolor{coverPinViolet}{HTML}{813BD0}
\definecolor{coverPinOrange}{HTML}{EA7929}
\definecolor{coverPinCyan}{HTML}{139BC7}
% A small clockwise turn flattens the paper journey without distorting objects.
\newcommand{\CoverFooterRotation}{-3}
\newcommand{\CoverScopeIconAt}[4]{%
  % #2 is the unchanged title node's north anchor. Its optical cap center
  % is about 5.6pt below that anchor at the retained 10.2pt title size.
  \begin{scope}[shift={(#1,#2)},yshift=-5.6pt]
    \CoverScopeSymbol{#3}{#4}%
  \end{scope}%
}
\newcommand{\CoverVerticalPin}[8][35mm]{%
  \draw[draw=#5,line width=0.65pt]
    (#8,#4) -- (#2,{#4+0.035}) -- (#2,{#3-0.010});%
  \filldraw[fill=#5,draw=white,line width=0.35pt]
    (#2,{#3-0.010}) circle (2.6pt);%
  \filldraw[fill=#5,draw=white,line width=0.35pt]
    (#8,#4) circle (1.6pt);%
  \node[anchor=north west,align=left,text width=#1,
    inner xsep=0pt,inner ysep=2pt,fill=none,draw=none]
    at ({#2+0.012},#3) {%
      \hyphenpenalty=10000\exhyphenpenalty=10000\relax
      {\fontfamily{droidserif}\fontsize{10.2}{12.2}\selectfont\bfseries
        \textcolor{coverInk}{#6}}\\[2.5pt]
      {\fontfamily{droidserif}\fontsize{8.2}{10.3}\selectfont
        \textcolor{coverMuted}{#7}}};%
}
\newcommand{\CoverReferencePinsCover}{%
  \AtPageLowerLeft{%
    \begin{tikzpicture}[overlay,x=\paperwidth,y=\paperheight]
      \clip (0,0) rectangle (1,1);
      \node[anchor=south west,inner sep=0pt] at (0,0) {%
        \includegraphics[width=\paperwidth,height=\paperheight]
          {figures/cover-variants/cover-bezier-reference-background-lowered.png}};
      % Keep the accepted lower ribbons without repainting their pixels.
      % Upper C-shaped framing is covered; a short fade avoids a crop seam.
      \fill[white] (0,0.265) rectangle (1,1);
      \path[fill=white,path fading=coverScopeFooterFade]
        (0,0.185) rectangle (1,0.265);
      % The blue outer world and the galactic work objects share one region.
      \begin{scope}[rotate around={\CoverFooterRotation:(0.09,0)}]
      \path[fill=coverPinViolet!4,fill opacity=0.45,
        draw=coverPinViolet!32,densely dotted,line width=0.5pt]
        (0.700,0.115)
        .. controls (0.700,0.185) and (0.765,0.290) .. (0.900,0.301)
        .. controls (0.980,0.320) and (1.055,0.280) .. (1.055,0.205)
        .. controls (1.055,0.120) and (0.880,0.070) .. (0.780,0.089)
        .. controls (0.735,0.091) and (0.715,0.098) .. (0.700,0.115)
        -- cycle;
      \end{scope}
    \end{tikzpicture}%
  }%
  \AtPageLowerLeft{%
    \begin{tikzpicture}[overlay,x=\paperwidth,y=\paperheight]
      \clip (0,0) rectangle (1,1);
      \begin{scope}[rotate around={\CoverFooterRotation:(0.09,0)},transform shape]
        \node[anchor=south west,inner sep=0pt,outer sep=0pt] at (0,0) {%
          \includegraphics[width=\paperwidth]
            {figures/cover-variants/cover-paper-journey-spaceflight-varied.png}};
      \end{scope}
    \end{tikzpicture}%
  }%
  \AtPageLowerLeft{%
    \begin{tikzpicture}[overlay,x=\paperwidth,y=\paperheight]
      % The scope arrow and its lettering follow one route below the worlds.
      % It encodes scope, not a strict hierarchy of agent ability.
      \begin{scope}[rotate around={\CoverFooterRotation:(0.09,0)}]
      \CoverScopeGradientArrow
      \path[decorate,decoration={text along path,
        text={|\fontfamily{droidserif}\fontsize{8.2}{10.0}\selectfont\color{coverInk!85}\CoverScopeLetterHalo|
          Expanding work scope and dependencies},
        text color=coverInk!85,raise=5pt,
        text align={align=right,right indent=30pt}}]
        (0.315,0.043)
        .. controls (0.485,0.052) and (0.760,0.096) .. (0.950,0.118);
      \end{scope}
      % Marker anchors follow the rotated artwork; keep the captions upright.
      % Place Workspace independently in the clear gap above the galaxy.
      \CoverScopeIconAt{0.074315}{0.220}{response}{coverPinBlue}
      \CoverScopeIconAt{0.275326}{0.235}{atomic}{coverPinViolet}
      \CoverScopeIconAt{0.46773056}{0.26825}{multi}{coverPinOrange}
      \CoverScopeIconAt{0.63219566}{0.28965152}{workflow}{coverPinCyan}
      \CoverScopeIconAt{0.78666783}{0.32837901}{workspace}{coverPinViolet}
      \CoverVerticalPin[36mm]{0.097315}{0.220}{0.107852}{coverPinBlue}
        {Conversation Level}{Interpret evidence\\Produce answers}{0.097315}
      \CoverVerticalPin[38mm]{0.298326}{0.235}{0.118738}{coverPinViolet}
        {Atomic Action Level}{Edit a local object\\Verify the change}{0.298326}
      \CoverVerticalPin[32mm]{0.49073056}{0.26825}{0.143240}{coverPinOrange}
        {Multi-step Level}{Dependent actions\\Complete an objective}{0.435175}
      \CoverVerticalPin[33mm]{0.65519566}{0.28965152}{0.177102}{coverPinCyan}
        {Workflow Level}{Coordinate stages\\and handoffs}{0.612712}
      % Keep the complete Workspace caption in the gap above the galaxy.
      % Its slightly leftward placement also clears the uppermost small planet.
      \CoverVerticalPin[37mm]{0.80966783}{0.32837901}{0.230740}{coverPinViolet}
        {\contourlength{1.0pt}\contour{white}{Workspace Level}}{\contourlength{1.4pt}\contour{white}{Connect related objects}\\\contour{white}{Track dependencies}}{0.788426}
    \end{tikzpicture}%
  }%
}


==> figures/cover-variants/cover-scope-gradient.tex <==
% Vector-only semantic route; called inside x=\paperwidth,y=\paperheight.
% The central shaft is an axial PDF shading clipped to a narrow Bezier band.
\usetikzlibrary{arrows.meta}
\definecolor{coverScopeGradientCobalt}{HTML}{2863BD}
\definecolor{coverScopeGradientTeal}{HTML}{169DA7}
\definecolor{coverScopeGradientIndigo}{HTML}{6752BF}
\pgfdeclarehorizontalshading{coverScopeGradientFlow}{100bp}{%
  color(0bp)=(coverScopeGradientCobalt);
  color(25bp)=(coverScopeGradientCobalt);
  color(48bp)=(coverScopeGradientTeal);
  color(75bp)=(coverScopeGradientIndigo);
  color(100bp)=(coverScopeGradientIndigo)}

\newcommand{\CoverScopeGradientArrow}{%
  % The white separator stays readable wherever background ribbons cross it.
  \draw[draw=white,line width=4.1pt,line cap=round,
    -{Stealth[length=3.35mm,width=2.65mm]}]
    (0.315,0.043)
    .. controls (0.485,0.052) and (0.760,0.096) .. (0.950,0.118);
  % This short segment is the exact t=.970--1 split of the same cubic.
  % A native arrowhead keeps the point crisp; no shading extends past it.
  \draw[draw=coverScopeGradientIndigo,line width=2.2pt,line cap=butt,
    -{Stealth[length=3.0mm,width=2.2mm]}]
    (0.93267563,0.115962139)
    .. controls (0.93852350,0.11666020) and (0.94430000,0.11734000)
    .. (0.950,0.118);
  \begin{scope}
    \clip
      ([yshift=1.1pt]0.315,0.043)
      .. controls ([yshift=1.1pt]0.47990000,0.05173000)
        and ([yshift=1.1pt]0.74359450,0.09339150)
      .. ([yshift=1.1pt]0.93267563,0.115962139)
      -- ([yshift=-1.1pt]0.93267563,0.115962139)
      .. controls ([yshift=-1.1pt]0.74359450,0.09339150)
        and ([yshift=-1.1pt]0.47990000,0.05173000)
      .. ([yshift=-1.1pt]0.315,0.043)
      -- cycle;
    \shade[shading=coverScopeGradientFlow]
      (0.314,0.039) rectangle (0.933,0.120);
  \end{scope}
  \fill[coverScopeGradientCobalt] (0.315,0.043) circle (1.1pt);
}


==> figures/cover-variants/cover-workscope-symbols.tex <==
% Editable work-scope glyphs. Usage inside a TikZ picture:
% \begin{scope}[shift={(x,y)}]\CoverScopeSymbol{response}{coverPinBlue}\end{scope}
% Kinds: response, atomic, multi, workflow, workspace.
% Visible glyph height is 12.5pt including the 0.75pt stroke, with no badge.
% Per-kind scaling uses the actual glyph extent rather than an empty frame.
\newcommand{\CoverScopeFitresponse}{%
  \def\CoverScopeScale{35.6060606061}% 11.75pt / 0.33
  \def\CoverScopeOffsetY{0.005}%
}
\newcommand{\CoverScopeFitatomic}{%
  \def\CoverScopeScale{32.6388888889}% 11.75pt / 0.36
}
\newcommand{\CoverScopeFitmulti}{%
  \def\CoverScopeScale{26.7045454545}% 11.75pt / 0.44
}
\newcommand{\CoverScopeFitworkflow}{%
  \def\CoverScopeScale{26.7045454545}% 11.75pt / 0.44
  \def\CoverScopeOffsetY{0.02}%
}
\newcommand{\CoverScopeFitworkspace}{%
  \def\CoverScopeScale{26.7045454545}% 11.75pt / 0.44
  \def\CoverScopeOffsetX{-0.005}%
}
\newcommand{\CoverScopeSymbol}[2]{%
  \begingroup
  \def\CoverScopeOffsetX{0}%
  \def\CoverScopeOffsetY{0}%
  \csname CoverScopeFit#1\endcsname
  \begin{scope}[x=1pt,y=1pt,scale=\CoverScopeScale,
    draw=#2,line width=0.75pt,line cap=round,line join=round]
  \begin{scope}[shift={(\CoverScopeOffsetX,\CoverScopeOffsetY)}]
    \csname CoverScopeDraw#1\endcsname{#2}%
  \end{scope}%
  \end{scope}%
  \endgroup
}

% A reply card: one bounded answer with two short content lines.
\newcommand{\CoverScopeDrawresponse}[1]{%
  \draw[rounded corners=0.6pt]
    (-0.19,0.16) -- (0.19,0.16) -- (0.19,-0.10)
    -- (-0.06,-0.10) -- (-0.13,-0.17) -- (-0.13,-0.10)
    -- (-0.19,-0.10) -- cycle;
  \draw (-0.12,0.07) -- (0.11,0.07)
    (-0.12,-0.01) -- (0.05,-0.01);
}

% One local document, with a folded corner and a small edit stroke.
\newcommand{\CoverScopeDrawatomic}[1]{%
  \draw (-0.15,-0.18) -- (-0.15,0.18) -- (0.06,0.18)
    -- (0.15,0.09) -- (0.15,-0.18) -- cycle;
  \draw (0.06,0.18) -- (0.06,0.09) -- (0.15,0.09)
    (-0.08,0.02) -- (0.07,0.02);
  \path[draw=#1,fill=#1!20] (-0.06,-0.12) -- (-0.08,-0.16)
    -- (-0.04,-0.14) -- (0.13,0.03) -- (0.10,0.06) -- cycle;
}

% Three dependent actions, connected in an ordered chain.
\newcommand{\CoverScopeDrawmulti}[1]{%
  \draw (-0.13,-0.13) -- (-0.04,-0.02)
    (0.04,0.02) -- (0.13,0.13);
  \path[draw=#1,fill=#1!9,rounded corners=0.5pt]
    (-0.23,-0.22) rectangle (-0.10,-0.09)
    (-0.065,-0.065) rectangle (0.065,0.065)
    (0.10,0.09) rectangle (0.23,0.22);
}

% Three process stages and two handoffs, shown as a compact flow.
\newcommand{\CoverScopeDrawworkflow}[1]{%
  \draw (-0.03,0.14) -- (0.15,0.14) -- (0.15,0.04)
    (0.03,-0.02) -- (-0.15,-0.02) -- (-0.15,-0.12);
  \path[draw=#1,fill=#1!9,rounded corners=0.5pt]
    (-0.24,0.08) rectangle (-0.03,0.20)
    (0.03,-0.08) rectangle (0.24,0.04)
    (-0.24,-0.24) rectangle (-0.03,-0.12);
  \path[fill=#1,draw=none]
    (0.15,0.035) -- (0.12,0.075) -- (0.18,0.075) -- cycle
    (-0.15,-0.115) -- (-0.18,-0.075) -- (-0.12,-0.075) -- cycle;
}

% A shared workspace: several linked objects around one central object.
\newcommand{\CoverScopeDrawworkspace}[1]{%
  \draw (0,0) -- (-0.18,0.15) -- (0.17,0.17) -- (0,0)
    -- (0.19,-0.14) -- (-0.17,-0.17) -- (0,0);
  \path[draw=#1,fill=#1!10,rounded corners=0.4pt]
    (-0.055,-0.055) rectangle (0.055,0.055)
    (-0.23,0.10) rectangle (-0.13,0.20)
    (0.12,0.12) rectangle (0.22,0.22)
    (0.14,-0.19) rectangle (0.24,-0.09)
    (-0.22,-0.22) rectangle (-0.12,-0.12);
}

